Unconditional Image-Text Pair Generation with Multimodal Cross Quantizer

Although deep generative models have gained a lot of attention, most of the existing works are designed for unimodal generation. In this paper, we explore a new method for unconditional image-text pair generation. We design Multimodal Cross-Quantization VAE (MXQ-VAE), a novel vector quantizer for joint image-text representations, with which we discover that a joint image-text representation space is effective for semantically consistent image-text pair generation. To learn a multimodal semantic correlation in a quantized space, we combine VQ-VAE with a Transformer encoder and apply an input masking strategy. Specifically, MXQ-VAE accepts a masked image-text pair as input and learns a quantized joint representation space, so that the input can be converted to a unified code sequence, then we perform unconditional image-text pair generation with the code sequence. Extensive experiments show the correlation between the quantized joint space and the multimodal generation capability on synthetic and real-world datasets. In addition, we demonstrate the superiority of our approach in these two aspects over several baselines. The source code is publicly available at: https://github.com/ttumyche/MXQ-VAE.

==> tables/cub_flower_stage1_degree.tex <==
\begin{table}[hbt!]
\begin{adjustbox}{width=\textwidth,center} %{height=2.8cm,center}
\begin{tabular}{ccccccccc}
\toprule
    \multicolumn{1}{c}{Dataset} &
    \multicolumn{1}{c}{Degree} &
    \multicolumn{1}{c}{Models}  &
    \multicolumn{1}{c}{Degree 4} &
    \multicolumn{1}{c}{Degree 3} &
    \multicolumn{1}{c}{Degree 2} &
    \multicolumn{1}{c}{Degree 1} &
    \multicolumn{1}{c}{Degree 0} \\
    \midrule
    & & Only Sharing \boldmath{$C$}     &	0.939	&	0.704	&	0.516	&	0.321	&	0.131 \\
    & & \model w/o TC &	1.0	&	0.944	&	0.886	&	0.866 & 0.810 \\
    & 4 colors & \model w/o IM                  &	0.997	&	0.728	&	0.482	&	0.278	&	0.067 \\
    Flower & & \textbf{\model (Ours)}                          &	0.996	&	0.737	&	0.490	&	0.250	&	0.014 \\
    
    \cmidrule(lr){2-8}
    & & Only Sharing \boldmath{$C$}     & - &	0.959	&	0.675	&	0.426	&	0.158 \\
    & & \model w/o TC & - &	1.0	&	0.927	&	0.870	&	0.816 \\
    & 3 colors & \model w/o IM                  & - &	0.997	&	0.662	&	0.377	&	0.090 \\
    & & \textbf{\model (Ours)}                          & - &	0.999	&	0.660	&	0.339	&	0.019 \\
    
    \midrule
    
    & & Only Sharing \boldmath{$C$}     &	0.985	&	0.771	&	0.572	&	0.356	&	0.155 \\
    & & \model w/o TC &	1.0	&	0.948	&	0.894	&	0.825	&	0.748 \\
    & 4 colors & \model w/o IM                  &	0.998	&	0.833	&	0.645	&	0.424	&	0.181 \\
    CUB & & \textbf{\model (Ours)}                          &	0.995	&	0.749	&	0.515	&	0.292	&	0.083 \\
    
    \cmidrule(lr){2-8}
    & & Only Sharing \boldmath{$C$}     & - &	0.986	&	0.755	&	0.498	&	0.199 \\
    & & \model w/o TC & - &	1.0	&	0.938	&	0.864	&	0.772 \\
    & 3 colors & \model w/o IM                  & - &	0.998	&	0.806	&	0.559	&	0.248 \\
    & & \textbf{\model (Ours)}                          & - &	0.995	&	0.709	&	0.421	&	0.119 \\
    
    % \midrule
    % & Only Sharing \boldmath{$C$}     & - & - &	0.973	&	0.592	&	0.204\\
    % & \model (w/o text compression) & - & - & 1.0  & 0.875 & 0.785 \\
    % 2 colors & \model w/o IM   & - & - &	0.998	&	0.552	&	0.146 \\
    % & \textbf{\model (Ours)}                          & - & - &	0.999	&	0.503	&	0.033 \\
    
    % \midrule
    % & Only Sharing \boldmath{$C$}     & - & - & - &	0.959	&	0.212 \\
    % & \model (w/o text compression) & - & - & - &	1.0	&	0.755 \\
    % 1 color & \model w/o IM                & - & - & - &	0.998	&	0.113 \\
    % & \textbf{\model(Ours)}                          & - & - & - &	0.999	&	0.013 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Multimodal semantic correlation on the Flower and CUB Degree dataset}}
\label{tab:cub_flower_stage1}
\end{table}

==> tables/cub_stage1_degree.tex <==
\begin{table}[hbt!]
\begin{adjustbox}{width=\textwidth,center} %{height=2.8cm,center}
\begin{tabular}{cccccccc}
\toprule
    \multicolumn{1}{c}{Degree} &
    \multicolumn{1}{c}{Models}  &
    \multicolumn{1}{c}{Degree 4} &
    \multicolumn{1}{c}{Degree 3} &
    \multicolumn{1}{c}{Degree 2} &
    \multicolumn{1}{c}{Degree 1} &
    \multicolumn{1}{c}{Degree 0} \\
    \midrule
    & Only Sharing \boldmath{$C$}     &	0.985	&	0.771	&	0.572	&	0.356	&	0.155 \\
    & \model w/o TC &	1.0	&	0.948	&	0.894	&	0.825	&	0.748 \\
    4 colors & \model w/o IM                  &	0.998	&	0.833	&	0.645	&	0.424	&	0.181 \\
    & \textbf{\model (Ours)}                          &	0.995	&	0.749	&	0.515	&	0.292	&	0.083 \\
    
    \midrule
    & Only Sharing \boldmath{$C$}     & - &	0.986	&	0.755	&	0.498	&	0.199 \\
    & \model w/o TC & - &	1.0	&	0.938	&	0.864	&	0.772 \\
    3 colors & \model w/o IM                  & - &	0.998	&	0.806	&	0.559	&	0.248 \\
    & \textbf{\model (Ours)}                          & - &	0.995	&	0.709	&	0.421	&	0.119 \\
    
    % \midrule
    % & Only Sharing \boldmath{$C$}     & - & - &	0.988	&	0.667	&	0.235 \\
    % & \model (w/o text compression) & - & - &	1.0	&	0.912	&	0.779 \\
    % 2 colors & \model w/o IM   & - & - &	0.999	&	0.723	&	0.308 \\
    % & \textbf{\model (Ours)}                          & - & - &	0.996	&	0.613	&	0.159 \\
    
    % \midrule
    % & Only Sharing \boldmath{$C$}     & - & - & - &	0.98	&	0.241 \\
    % & \model (w/o text compression) & - & - & - &	1.0	&	0.790 \\
    % 1 color& \model w/o IM                & - & - & - &	0.998	&	0.321 \\
    % & \textbf{\model(Ours)}                          & - & - & - &	0.994	&	0.151 \\
    
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Multimodal semantic correlation on the CUB Degree dataset}
\label{tab:cub_degree}
\end{table}



% \begin{table}
% \begin{adjustbox}{width=\textwidth,center}
% \begin{tabular}{cccccccc}
% \toprule
%     \multicolumn{1}{c}{Degree} &
%     \multicolumn{1}{c}{Models}  &
%     \multicolumn{1}{c}{Degree 4} &
%     \multicolumn{1}{c}{Degree 3} &
%     \multicolumn{1}{c}{Degree 2} &
%     \multicolumn{1}{c}{Degree 1} &
%     \multicolumn{1}{c}{Degree 0} \\
%     \midrule
%     & Only Sharing \boldmath{$e$}     &	0.98506	&	0.771383	&	0.57226	&	0.356372	&	0.155353 \\
%     4 colors & \model (w/o text compression)               &	0.999787	&	0.948475	&	0.893851	&	0.825009	&	0.748481 \\
%     & \model (w/o input masking)                  &	0.998012	&	0.832992	&	0.645206	&	0.424193	&	0.180659 \\
%     & \textbf{\model (Ours)}                          &	0.994822	&	0.748598	&	0.514763	&	0.291566	&	0.08338 \\
%     \midrule
    
%     & Only Sharing \boldmath{$e$}     & - &	0.985612	&	0.75491	&	0.497852	&	0.198518 \\
%     3 colors & \model (w/o text compression)            & - &	0.999834	&	0.938373	&	0.863805	&	0.771763 \\
%     & \model (w/o input masking)                  & - &	0.998474	&	0.806139	&	0.558594	&	0.248447 \\
%     & \textbf{\model (Ours)}                          & - &	0.994997	&	0.709127	&	0.420563	&	0.118604 \\
%     \midrule
    
%     & Only Sharing \boldmath{$e$}     & - & - &	0.988383	&	0.667361	&	0.234519 \\
%     2 colors & \model (w/o text compression)               & - & - &	0.999957	&	0.911697	&	0.779163 \\
%     & \model (w/o input masking)   & - & - &	0.998775	&	0.722912	&	0.308249 \\
%     & \textbf{\model (Ours)}                          & - & - &	0.99586	&	0.613498	&	0.159176 \\
%     \midrule
    
%     & Only Sharing \boldmath{$e$}     & - & - & - &	0.979693	&	0.2406 \\
%     1 color & \model (w/o text compression)            & - & - & - &	0.999959	&	0.790306 \\
%     & \model (w/o input masking)                & - & - & - &	0.998158	&	0.321264 \\
%     & \textbf{\model(Ours)}                          & - & - & - &	0.994437	&	0.150655 \\
    
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{Multimodal semantic correlation on the CUB Degree dataset}
% \label{tab:cub_degree}
% \end{table}

==> tables/cub_stage2.tex <==
% \begin{table}[hbt!]
% \begin{adjustbox}{width=\textwidth,center}
% \begin{tabular}{ccccccccc}
% \toprule
%     \multirow{3}{*}{Models}  &
%     \multicolumn{4}{c}{Label-based}  &
%     \multicolumn{4}{c}{CLIP-based}  \\
%     \cmidrule(lr){2-5}
%     \cmidrule(lr){6-9}
%     & Word matching &  & Sentence similarity & & Word matching & & Sentence similarity & \\ 
%     \cmidrule(lr){3-5}
%     \cmidrule(lr){7-9}
%     & accuracy & Top-1 & Top-5 & Top-10 & accuracy & Top-1 & Top-5 & Top-10 \\ 
%     \midrule
%     I\&T\_VQ                                        & - & 0.942 & 0.931 & 0.925 & - & 0.942 & 0.931 & 0.925 \\
%     T\&I\_VQ                                        & - & 0.925 & 0.912 & 0.903 & - & 0.925 & 0.912 & 0.903 \\
%     I\_T\_VQ                                        & - & 0.92 & 0.91 & 0.904 & - & 0.92 & 0.91 & 0.904 \\
%     T\_I\_VQ                                        & - & 0.941 & 0.929 & 0.922 & - & 0.941 & 0.929 & 0.922 \\
%     I(VQ)\_T(Embd)                                  & - & 0.96 & 0.949 & 0.942 & - & 0.96 & 0.949 & 0.942 \\
%     T(Embd)\_I(VQ)                                  & - & 0.934 & 0.919 & 0.911 & - & 0.934 & 0.919 & 0.911 \\
%     \model (w/o text compression)                   & - & 0.964 & 0.955 & 0.949 & - & 0.964 & 0.955 & 0.949 \\
%     \textbf{\model (Ours)}                          & - & \textbf{0.967} & \textbf{0.958} & \textbf{0.952} & - & \textbf{0.967} & \textbf{0.958} & \textbf{0.952} \\
    
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{Semantic consistency of the generated image-text pairs on CUB.}
% \label{tab:cub_stage2}
% \end{table}

\begin{table}[hbt!]
\begin{center}
\begin{tabular}{ccccc}
\toprule
    \multirow{2}{*}{Models}  &
    \multirow{2}{*}{Word matching}  &
    \multicolumn{3}{c}{Sentence Similarity ($\uparrow$)} \\
    \cmidrule(lr){3-5}
    & accuracy & Top-1 & Top-5 & Top-10 \\ 
    \midrule
    % Oxford-102                                    & 0.999 & 0.963 & 0.962 & - \\
    I\&T\_VQ                                        & - & 0.942 & 0.931 & 0.925 \\
    T\&I\_VQ                                        & - & 0.925 & 0.912 & 0.903 \\
    I\_T\_VQ                                        & - & 0.92 & 0.91 & 0.904 \\
    T\_I\_VQ                                        & - & 0.941 & 0.929 & 0.922 \\
    I(VQ)\_T(Embd)                                  & - & 0.96 & 0.949 & 0.942 \\
    T(Embd)\_I(VQ)                                  & - & 0.934 & 0.919 & 0.911 \\
    \model (w/o text compression)                   & - & 0.964 & 0.955 & 0.949 \\
    % I\&T\_VQ\_TBERT                               & 0.968 & 0.956 & 0.95 \\
    % T\&I\_VQ\_TBERT                               & 0.792 & 0.762 & 0.744 \\
    Joint GAN \citep{shimanuki2019joint} $^\ast$    & - & 0.832 & 0.813 & 0.802 \\
    \textbf{\model (Ours)}                          & - & \textbf{0.967} & \textbf{0.958} & \textbf{0.952} \\
    
\bottomrule
\end{tabular}
\end{center}
\caption{Semantic consistency of the generated image-text pairs on CUB.}
% * means we measure the score with reported image-text pairs in Joint GAN \citep{shimanuki2019joint}.
\label{tab:flower_stage2_all}
\end{table}

==> tables/flower_stage1_degree.tex <==
\begin{table}[hbt!]
\begin{adjustbox}{width=\textwidth,center} %{height=2.8cm,center}
\begin{tabular}{cccccccc}
\toprule
    \multicolumn{1}{c}{Degree} &
    \multicolumn{1}{c}{Models}  &
    \multicolumn{1}{c}{Degree 4} &
    \multicolumn{1}{c}{Degree 3} &
    \multicolumn{1}{c}{Degree 2} &
    \multicolumn{1}{c}{Degree 1} &
    \multicolumn{1}{c}{Degree 0} \\
    \midrule
    & Only Sharing \boldmath{$C$}     &	0.939	&	0.704	&	0.516	&	0.321	&	0.131 \\
    & \model w/o TC &	1.0	&	0.944	&	0.886	&	0.866 & 0.810 \\
    4 colors & \model w/o IM                  &	0.997	&	0.728	&	0.482	&	0.278	&	0.067 \\
    & \textbf{\model (Ours)}                          &	0.996	&	0.737	&	0.490	&	0.250	&	0.014 \\
    
    \midrule
    & Only Sharing \boldmath{$C$}     & - &	0.959	&	0.675	&	0.426	&	0.158 \\
    & \model w/o TC & - &	1.0	&	0.927	&	0.870	&	0.816 \\
    3 colors & \model w/o IM                  & - &	0.997	&	0.662	&	0.377	&	0.090 \\
    & \textbf{\model (Ours)}                          & - &	0.999	&	0.660	&	0.339	&	0.019 \\
    
    % \midrule
    % & Only Sharing \boldmath{$C$}     & - & - &	0.973	&	0.592	&	0.204\\
    % & \model (w/o text compression) & - & - & 1.0  & 0.875 & 0.785 \\
    % 2 colors & \model w/o IM   & - & - &	0.998	&	0.552	&	0.146 \\
    % & \textbf{\model (Ours)}                          & - & - &	0.999	&	0.503	&	0.033 \\
    
    % \midrule
    % & Only Sharing \boldmath{$C$}     & - & - & - &	0.959	&	0.212 \\
    % & \model (w/o text compression) & - & - & - &	1.0	&	0.755 \\
    % 1 color & \model w/o IM                & - & - & - &	0.998	&	0.113 \\
    % & \textbf{\model(Ours)}                          & - & - & - &	0.999	&	0.013 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Multimodal semantic correlation on the Flower Degree dataset}
\label{tab:flower_degree}
\end{table}

% \begin{table}
% \begin{adjustbox}{width=\textwidth,center}
% \begin{tabular}{cccccccc}
% \toprule
%     \multicolumn{1}{c}{Degree} &
%     \multicolumn{1}{c}{Models}  &
%     \multicolumn{1}{c}{Degree 4} &
%     \multicolumn{1}{c}{Degree 3} &
%     \multicolumn{1}{c}{Degree 2} &
%     \multicolumn{1}{c}{Degree 1} &
%     \multicolumn{1}{c}{Degree 0} \\
%     \midrule
%     & Only Sharing \boldmath{$e$}     &	0.939395	&	0.703876	&	0.515596	&	0.320516	&	0.131098 \\
%     4 colors & \model (w/o text compression)               &	0.9991	&	0.944281	&	0.885943	&	0.865757	&	0.810205 \\
%     & \model (w/o input masking)                  &	0.9967	&	0.72761	&	0.482314	&	0.277952	&	0.067186 \\
%     & \textbf{\model (Ours)}                          &	0.995899	&	0.736937	&	0.489504	&	0.249965	&	0.013956 \\
%     \midrule
    
%     & Only Sharing \boldmath{$e$}     & - &	0.958629	&	0.674572	&	0.426065	&	0.157822 \\
%     3 colors & \model (w/o text compression)            & - &	0.999696	&	0.926663	&	0.869964	&	0.816282 \\
%     & \model (w/o input masking)                  & - &	0.997247	&	0.661756	&	0.376774	&	0.089947 \\
%     & \textbf{\model (Ours)}                          & - &	0.998792	&	0.660342	&	0.339463	&	0.018571 \\
%     \midrule
    
%     & Only Sharing \boldmath{$e$}     & - & - &	0.973216	&	0.591757	&	0.204148 \\
%     2 colors & \model (w/o text compression)               & - & - & 0.999929268  &0.875160976 &0.784871138 \\
%     & \model (w/o input masking)   & - & - &	0.998146748	&	0.551588618	&	0.146222358 \\
%     & \textbf{\model (Ours)}                          & - & - &	0.9987	&	0.503229	&	0.032602 \\
%     \midrule
    
%     & Only Sharing \boldmath{$e$}     & - & - & - &	0.958669	&	0.211697 \\
%     1 color & \model (w/o text compression)            & - & - & - &	0.999989	&	0.754645 \\
%     & \model (w/o input masking)                & - & - & - &	0.997808	&	0.11304 \\
%     & \textbf{\model(Ours)}                          & - & - & - &	0.99884	&	0.012986 \\
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{Multimodal semantic correlation on the Flower Degree dataset}
% \label{tab:flower_degree}
% \end{table}

==> tables/flower_stage2.tex <==
% \begin{table}[hbt!]
% \begin{center}
% \begin{tabular}{ccccc}
% \toprule
%     \multirow{2}{*}{Models}  &
%     \multirow{2}{*}{Word matching}  &
%     \multicolumn{3}{c}{Sentence Similarity ($\uparrow$)} \\
%     \cmidrule(lr){3-5}
%     & accuracy & Top-1 & Top-5 & Top-10 \\ 
%     \midrule
%     % Oxford-102                                    & 0.999 & 0.963 & 0.962 & - \\
%     I\&T\_VQ                                        & - & 0.942 & 0.931 & 0.925 \\
%     T\&I\_VQ                                        & - & 0.925 & 0.912 & 0.903 \\
%     I\_T\_VQ                                        & - & 0.92 & 0.91 & 0.904 \\
%     T\_I\_VQ                                        & - & 0.941 & 0.929 & 0.922 \\
%     I(VQ)\_T(Embd)                                  & - & 0.96 & 0.949 & 0.942 \\
%     T(Embd)\_I(VQ)                                  & - & 0.934 & 0.919 & 0.911 \\
%     \model (w/o text compression)                   & - & 0.964 & 0.955 & 0.949 \\
%     % I\&T\_VQ\_TBERT                               & 0.968 & 0.956 & 0.95 \\
%     % T\&I\_VQ\_TBERT                               & 0.792 & 0.762 & 0.744 \\
%     Joint GAN \citep{shimanuki2019joint} $^\ast$    & - & 0.832 & 0.813 & 0.802 \\
%     \textbf{\model (Ours)}                          & - & \textbf{0.967} & \textbf{0.958} & \textbf{0.952} \\
    
% \bottomrule
% \end{tabular}
% \end{center}
% \caption{Semantic consistency of the generated image-text pairs on Flower.}
% % * means we measure the score with reported image-text pairs in Joint GAN \citep{shimanuki2019joint}.
% \label{tab:flower_stage2_all}
% \end{table}


\begin{table}[hbt!]
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{ccccccccc}
\toprule
    \multirow{3}{*}{Models}  &
    \multicolumn{4}{c}{CUB}  &
    \multicolumn{4}{c}{Flower}  \\
    \cmidrule(lr){2-5}
    \cmidrule(lr){6-9}
    & Word matching &  & Sentence similarity & & Word matching & & Sentence similarity & \\ 
    \cmidrule(lr){3-5}
    \cmidrule(lr){7-9}
    & accuracy & Top-1 & Top-5 & Top-10 & accuracy & Top-1 & Top-5 & Top-10 \\ 
    \midrule
    I\&T\_VQ                                        & - & 0.942 & 0.931 & 0.925 & - & 0.942 & 0.931 & 0.925 \\
    T\&I\_VQ                                        & - & 0.925 & 0.912 & 0.903 & - & 0.925 & 0.912 & 0.903 \\
    I\_T\_VQ                                        & - & 0.92 & 0.91 & 0.904 & - & 0.92 & 0.91 & 0.904 \\
    T\_I\_VQ                                        & - & 0.941 & 0.929 & 0.922 & - & 0.941 & 0.929 & 0.922 \\
    I(VQ)\_T(Embd)                                  & - & 0.96 & 0.949 & 0.942 & - & 0.96 & 0.949 & 0.942 \\
    T(Embd)\_I(VQ)                                  & - & 0.934 & 0.919 & 0.911 & - & 0.934 & 0.919 & 0.911 \\
    \model (w/o text compression)                   & - & 0.964 & 0.955 & 0.949 & - & 0.964 & 0.955 & 0.949 \\
    Joint GAN \citep{shimanuki2019joint} $^\ast$    & - & 0.832 & 0.813 & 0.802 & - & 0.832 & 0.813 & 0.802 \\
    \textbf{\model (Ours)}                          & - & \textbf{0.967} & \textbf{0.958} & \textbf{0.952} & - & \textbf{0.967} & \textbf{0.958} & \textbf{0.952} \\
    
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Semantic consistency of the generated image-text pairs on CUB and Flower.}
% * means we measure the score with reported image-text pairs in Joint GAN \citep{shimanuki2019joint}.
\label{tab:flower_stage2}
\end{table}

==> tables/mnist_stage1_degree_all.tex <==
\begin{table}[hbt!]
\begin{adjustbox}{height=2cm,center} %{width=\textwidth,center} %
\begin{tabular}{cccccccc}
\toprule
    \multicolumn{1}{c}{Degree} &
    \multicolumn{1}{c}{Models}  &
    \multicolumn{1}{c}{Degree 4} &
    \multicolumn{1}{c}{Degree 3} &
    \multicolumn{1}{c}{Degree 2} &
    \multicolumn{1}{c}{Degree 1} &
    \multicolumn{1}{c}{Degree 0} \\
    \midrule
    & Only Sharing \boldmath{$C$}     & 0.486 & 0.443 & 0.394 & 0.358 & 0.315 \\
    & \model w/o TC   &	1.0	&	0.975	&	0.951	&	0.929	&	0.906 \\
    Quad4 & \model w/o IM                 &	0.896	&	0.802	&	0.698	&	0.595	&	0.498 \\
    &  \textbf{\model (Ours)}                         &	 0.969	&	 0.729	&	 0.489	&	 0.248	&	 0.009 \\
    
    \midrule
    & Only Sharing \boldmath{$C$}     & - & 0.713 & 0.64 & 0.558 & 0.483 \\
    & \model w/o TC   & - &	1.0	&	0.968	&	0.943	&	0.909 \\
    Quad3 & \model w/o IM                  & - &	0.999	&	0.862	&	0.714	&	0.564 \\
    &  \textbf{\model (Ours)}                          &	-	&	 0.997	&	 0.663	&	 0.334	&	 0.012 \\
    
    % \midrule
    % & Only Sharing \boldmath{$C$}     & - & - & 0.905 & 0.776 & 0.65 \\
    % & \model (w/o text compression)               & - & - &	1.0	&	0.969	&	0.935 \\
    % Quad2 & \model w/o IM   & - & - &	0.999	&	0.808	&	0.603 \\
    % &  \model (Ours)}                         &	-	&	-	&	0.997	&	0.494	&	0.005 \\
    
    % \midrule
    % & Only Sharing \boldmath{$C$}     & - & - & - & 1.0 & 0.772 \\
    % & \model (w/o text compression)            & - & - & - &	1.0	&	0.942 \\
    % Quad1& \model w/o IM                & - & - & - &	1.0	&	0.659\\
    % &  \model(Ours)}                          &	-	&	-	&	-	&	0.997	&	0.000 \\
    
    % \midrule
    % & Only Sharing \boldmath{$C$}     & - & - & - & 1.0 & 0.840 \\
    % & \model (w/o text compression)            & - & - & - &	1.0	&	0.935 \\
    % Single & \model w/o IM                & - & - & - &	1.0	&	0.639\\
    % &  \model (Ours)}                          &	-	&	-	&	-	&	0.997	&	0.000 \\
    
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{\textbf{Multimodal semantic correlation on the Caption MNIST Degree dataset} \\ 
The scores close to 1.0, 0.75, 0.5, 0.25, and 0.0 on Quad4 and 1.0, 0.66, 0.33, and 0.0 on Quad3 are better. In general, our approach shows the best approximation performance.}
\label{tab:mnist_degree_all}
\end{table}

% \begin{table} %[hbt!]
% \begin{adjustbox}{height=3.5cm,center}
% \begin{tabular}{cccccccc}
% \toprule
%     \multicolumn{1}{c}{Degree} &
%     \multicolumn{1}{c}{Models}  &
%     \multicolumn{1}{c}{Degree 4} &
%     \multicolumn{1}{c}{Degree 3} &
%     \multicolumn{1}{c}{Degree 2} &
%     \multicolumn{1}{c}{Degree 1} &
%     \multicolumn{1}{c}{Degree 0} \\
%     \midrule
%     & Only Sharing \boldmath{$C$}     & 0.486 & 0.443 & 0.394 & 0.358 & 0.315 \\
%     % Quad4 & \model (w/o text compression)               &	0.99995	&	0.97535	&	0.9507	&	0.92875	&	0.9062 \\
%     Quad4 & \model w/o IM                 &	0.8956	&	0.80205	&	0.6979	&	0.59495	&	0.49825 \\
%     &  \model (Ours)}                          &	0.9688	&	0.7285	&	0.489	&	0.2484	&	0.00945 \\
    
%     \midrule
%     & Only Sharing \boldmath{$C$}     & - & 0.713 & 0.64 & 0.558 & 0.483 \\
%     % Quad3 & \model (w/o text compression)            & - &	1	&	0.967733	&	0.9432	&	0.9088 \\
%     Quad3 & \model w/o IM                  & - &	0.998867	&	0.862067	&	0.7144	&	0.563867 \\
%     &  \model (Ours)}                          &	-	&	0.9966	&	0.663333	&	0.3342	&	0.011733 \\
    
%     \midrule
%     & Only Sharing \boldmath{$C$}     & - & - & 0.905 & 0.776 & 0.65 \\
%     % Quad2 & \model (w/o text compression)               & - & - &	1	&	0.9689	&	0.9354 \\
%     Quad2 & \model w/o IM   & - & - &	0.9994	&	0.8079	&	0.6025 \\
%     &  \model (Ours)}                         &	-	&	-	&	0.9965	&	0.4943	&	0.005 \\
    
%     \midrule
%     & Only Sharing \boldmath{$C$}     & - & - & - & 1.0 & 0.772 \\
%     % Quad1 & \model (w/o text compression)            & - & - & - &	1	&	0.9418 \\
%     Quad1& \model w/o IM                & - & - & - &	1	&	0.6592\\
%     &  \model(Ours)}                          &	-	&	-	&	-	&	0.9974	&	0.0 \\
    
%     \midrule
%     & Only Sharing \boldmath{$C$}     & - & - & - & 1.0 & 0.84 \\
%     % Single & \model (w/o text compression)            & - & - & - &	0.9998	&	0.9352 \\
%     Single & \model w/o IM                & - & - & - &	1	&	0.6392\\
%     &  \model (Ours)}                          &	-	&	-	&	-	&	0.9972	&	0.0 \\
    
% \bottomrule
% \end{tabular}
% \end{adjustbox}
% \caption{Multimodal semantic correlation on the Caption MNIST Degree dataset}
% \label{tab:mnist_degree_all}
% \end{table}

==> tables/mnist_stage1_degree_mse.tex <==
\begin{table}
\begin{adjustbox}{width=\textwidth,center}
\begin{tabular}{cccccccc}
\toprule
    \multicolumn{1}{c}{Degree} &
    \multicolumn{1}{c}{Models}  &
    \multicolumn{1}{c}{Degree 4} &
    \multicolumn{1}{c}{Degree 3} &
    \multicolumn{1}{c}{Degree 2} &
    \multicolumn{1}{c}{Degree 1} &
    \multicolumn{1}{c}{Degree 0} \\
    \midrule
    & Only Sharing \boldmath{$e$}     &	0.050088	&	0.050088	&	0.050088	&	0.050088	&	0.050088 \\
    Quad4 & \model (w/o text compression)               &	0.067077	&	0.067139	&	0.06718	&	0.06727	&	0.067414 \\
    & \model (w/o input masking)                  &	0.068589	&	0.069125	&	0.069532	&	0.070155	&	0.071158 \\
    & \textbf{\model (Ours)}                          &	0.069774	&	0.069776	&	0.069719	&	0.069732	&	0.069742 \\
    \midrule
    
    & Only Sharing \boldmath{$e$}     & - &	0.037646	&	0.037646	&	0.037646	&	0.037646 \\
    Quad3 & \model (w/o text compression)            & - &	0.050586	&	0.050664	&	0.050674	&	0.050804 \\
    & \model (w/o input masking)                  & - &	0.050849	&	0.051164	&	0.051489	&	0.052209 \\
    & \textbf{\model (Ours)}                          &	-	&	0.052501	&	0.052498	&	0.052542	&	0.052569 \\
    \midrule
    
    & Only Sharing \boldmath{$e$}     & - & - &	0.024866	&	0.024866	&	0.024866 \\
    Quad2 & \model (w/o text compression)               & - & - &	0.033951	&	0.034086	&	0.0342 \\
    & \model (w/o input masking)   & - & - &	0.033525	&	0.033695	&	0.033839 \\
    & \textbf{\model (Ours)}                         &	-	&	-	&	0.035068	&	0.035045	&	0.035074 \\
    \midrule
    
    & Only Sharing \boldmath{$e$}     & - & - & - &	0.01222	&	0.01222 \\
    Quad1 & \model (w/o text compression)            & - & - & - &	0.016765	&	0.016877 \\
    & \model (w/o input masking)                & - & - & - &	0.016587	&	0.016663\\
    & \textbf{\model(Ours)}                          &	-	&	-	&	-	&	0.017208	&	0.017248 \\
    \midrule
    
    & Only Sharing \boldmath{$e$}     & - & - & - &	0.012403	&	0.012403 \\
    Single & \model (w/o text compression)            & - & - & - &	0.016496	&	0.163606 \\
    & \model (w/o input masking)                & - & - & - &	0.015971	&	0.021517\\
    & \textbf{\model (Ours)}                          &	-	&	-	&	-	&	0.017631	&	0.017633 \\
    
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Image reconstruction on the Caption MNIST Degree dataset}
\label{tab:mnist_degree_mse}
\end{table}
